A Model for Multi-Agent Heterogeneous Interaction Problems

We introduce a model for multi-agent interaction problems to understand how a heterogeneous team of agents should organize its resources to tackle a heterogeneous team of attackers. This model is inspired by how the human immune system tackles a diverse set of pathogens. The key property of this model is a ``cross-reactivity'' kernel which enables a particular defender type to respond strongly to some attacker types but weakly to a few different types of attackers. We show how due to such cross-reactivity, the defender team can optimally counteract a heterogeneous attacker team using very few types of defender agents, and thereby minimize its resources. We study this model in different settings to characterize a set of guiding principles for control problems with heterogeneous teams of agents, e.g., sensitivity of the harm to sub-optimal defender distributions, and competition between defenders gives near-optimal behavior using decentralized computation of the control. We also compare this model with existing approaches including reinforcement-learned policies, perimeter defense, and coverage control.

==> heterogeneity.tex <==
% !TEX root = ./root.tex

\section{Heterogeneity and Non Uniform Cross-Reactivity}
\label{s:heterogeneity}
\cite{Mitra-HeterogeneityBandit}
The cross reactivity function is intuitively easier to understand the when state space is in Euclidean. When agents are in this space, the Euclidean distance function is intuitive where agents close in distance can react with high probability and vice versa. In this section, we provide an example of how the cross reactivity function can be thought of in a heterogeneous space, where the distance between types is dependent on the agent's capabilities. 

Consider the scenario where 4 different types of agents interact according to~\cref{fig:heterogeneity}. 

\begin{figure}[!htpb]
    \centering
    % \includegraphics[width=0.49\linewidth]{case0_nonunif}
    % \includegraphics[width=0.49\linewidth]{heterogeneity}
    \includegraphics[width=0.49\linewidth]{nonunif}
    \includegraphics[width=0.49\linewidth]{nonunif_sigs}
    % \includegraphics[width=0.49\linewidth]{nonunif3}
    \caption{}
    \label{fig:heterogeneity}
\end{figure}

==> kf.tex <==
% !TEX root = ./root.tex

\section{Estimating an unknown attacker distribution}
\label{s:KF}

We are next interested in understanding scenarios when the attacker distribution $Q_a$ is not known to the defenders and the distribution changes over time. We will change the attacker distribution in two ways: (a) different types of attackers arrive as time progresses, and (b) attackers shift in the shape-space by changing their capabilities. These are both motivated by the setting where an adversary reallocates the composition of the attacker team after observing a few iterations of the interaction. Our strategy will be to estimate the changing attacker distribution $Q_a(t)$ and use this estimate to calculate a new optimal distribution for defenders $P_d^*(t)$ at each time step. Interactions, both successful or not, provide us observations of the attacker types $a$ that exist in the environment, and thereby the distribution $Q_a(t)$.

Our model for how attackers proliferate enables us to estimate their distribution as follows. Let us first assume that $Q_a$ is unknown to the defenders but it is stationary, i.e., it does not change with time. From~\cref{s:problem}, the expected number of attackers is $m_a(t)$ and it grows as $m_a(t) = m_a(0) e^{\nu_a t}$. We assume that $m_a(0) = 1$ for attackers $a$ that were sampled from $Q_a$. If we can estimate $\hat m_a(0)$ then we can think of the attackers corresponding to it as sampled from $Q_a$ and obtain an estimate $\hat Q_a$.

Let us arrange all the attackers into a vector $x(t) \in \reals^{m_a(t)}$ which will be the state of our filter. We will assume that $x_i \sim N(\mu_i, \s_i)$ for $i \leq m_a(t)$ and we receive observations $y_i = c x_i + \xi$ where $c$ is a Boolean that indicates if this specific attacker interacted with the defenders and $\xi \sim N(0, \s_\xi^2)$ is Gaussian noise. We can update $\mu_i^+ = \mu_i + k (y_i - c \mu_i)$ and $(\s_i^+)^2 = (1 - k c) \s_i^2$ using the Kalman gain $k = \s_i^2 c/(c^2 \s_i^2 + \s_\xi^2)$. The growth rate can now be estimated as $\hat{\nu}_i = \log (\mu_i^+/\mu_i)$. Since there are multiple attackers for each type, we average the estimates
\[
        \hat{\mu}_a(t) = \f{\sum_{i=1}^{m_a(t)} \ind{\text{type }(x_i) = a} \mu_i}{\sum_{i=1}^{m_a(t)} \ind{\text{type }(x_i) = a}},
\]
and similarly for $\hat{\nu}_a$ to get $\hat{Q}_a(t) = \hat{\mu}_a e^{- \hat{\nu}_a t}$. Let us emphasize that the number of attackers $m_a(t)$ (and therefore the dimensionality of the state $x$ of the filter) grows with time but this can be handled in the implementation easily. As written, this filter runs independently for each attacker (and therefore each attacker type) but it is easy to incorporate a known model of the correlations between the growth rates $\nu_a$ of different attacker types. Given the estimate of $\hat{Q}_a(t)$, we recalculate the optimal defender distribution $P_d^*(t)$ by minimizing~\cref{eq:harm} at each instant.

\cref{fig:kf_stationary} discusses simulation experiments using an unknown and stationary $Q_a$ using the above filter. At the beginning of each episode, we sample a new set of attackers from $Q_a$ and within every episode $0 \leq t \leq T$, we sample defenders from $P_d^*(t)$ that is calculated using the $\hat{Q}_a(t)$ estimated by the filter. We initialize $\hat{Q}_a(0)$ to be uniform and $P_d^*(0)$ using~\cref{eq:harm}. The episode ends at a random time $T$ when the final attacker is recognized by the defense and the total harm of that episode is the harm incurred until all attackers are recognized. The estimate of $\hat{Q}_a$ is initialized to its final value $\hat{Q}_a(T)$ from the previous episode. In other words, defenders get multiple opportunities to estimate the attacker distribution. \emph{Attacker types} can be different across episodes but the attacker distribution $Q_a$ is the same across episodes. We run each experiment for 100 episodes.

\begin{figure}[!htpb]
    \centering
    % \includegraphics[width=\linewidth]{c2-harms}
    % \includegraphics[width=\linewidth]{case2}
    \includegraphics[width=0.49\linewidth]{c2-wd}
    \includegraphics[width=0.49\linewidth]{c2-harms}
    \includegraphics[width=0.49\linewidth]{c2-qa}
    \includegraphics[width=0.49\linewidth]{c2-pd}
    \caption{Estimating an unknown and stationary attacker distribution.
    %
    \textbf{Top:} We plot the $W_1$ metric between the ground truths $Q_a, P_d^*$ against estimates $\hat{Q}_a$, $P_d$ over episodes.
    % between the true $Q_a$ and the estimated $\hat{Q}_a$ over the course of the experiment to observe the accuracy of the estimation.  HD is also calculated between the optimal $P_d^*$ and the $P_d$ found from $\hat{Q}_a$. 
    On the right we compare $P_d^*$ analytical harm and empirical harms' means and standard deviations as the defenders gain a better estimation of $Q_a$.
    \textbf{Bottom:}
    We show the final $\hat{Q}_a$ estimated at the end of 100 episodes (orange) against the actual $Q_a$ (blue) in the left plot. On the right, we have ground truth $P_d^*(Q_a)$ and estimated $P_d(\hat{Q}_a)$. 
    }
    \label{fig:kf_stationary}
\end{figure}

\cref{fig:kf_stationary} (top left) shows that the Wasserstein distance between the true $Q_a$ and the estimated $\hat{Q}_a$ decreases with the number of episodes. Due to the stochasticity of the observations, the filter estimates an approximate value $\hat Q_a$ which has a higher coefficient of variation $\k$ than that of the true $Q_a$ (seen as shorter spikes in~\cref{fig:kf_stationary} bottom left). Note that even if the estimation procedure does not recover the true $Q_a$ the corresponding optimal defender distribution $P_d^*(\hat Q_a)$ is close to $P_d^*(Q_a)$ in terms of the Wasserstein metric. This has important practical implications: we can obtain near-minimal harm even with incomplete information of the attacker team's constitution for large multi-agent problems (this simulation has 1000 attackers and 1000 defenders). The fundamental reason for this is cross-reactivity $f_{d,a}$; a given defender type can counter, even if sub-optimally, many other attacker types.

% The resulting $P_d(\hat{Q}_a)$ moves towards $P_d^*$. Empirical harm incurred by the defenders using the estimated $\hat{Q}_a$ (orange,~\cref{eq:Fbar}) converges to the optimal harm as if $Q_a$ was known perfectly (blue) as the defenders see more episodes. 
% The large spikes in the right plot are due to noisy observations resulting from suboptimal defender distributions which further result in an inaccurate estimate of $\hat{Q}_a$. But once $\hat{Q}_a$ stabilizes (around 30 episodes), the empirical harm mean is approximately equal to the analytical harm.

% In~\cref{fig:case2-harms} (A), we see similarly to~\cref{fig:case1} that the $\text{TV}(Q_a, \hat{Q}_a)$ decreases over time as the estimate $\hat{Q}_a$ get close to the true $Q_a$. Although the estimate is not exact as shown by the curve stabilizing at around 0.4 $\text{TV}(Q_a, \hat{Q}_a)$ but the harm caused to $P_d$ is close the harm caused to $P_d^*$. Why might this be the case?

% It can be seen that due to cross-reactivity, the optimal defender distribution is spiked according to the cross-reactive width, $\sigma$, and uniformly covers the perimeter. This characteristic of the defensive distribution is an important consequence for when we have different samples from the same attacker distribution. Each episode, the defense will observe a slightly different spectrum of attackers because of the stochasticity of observations and the resulting calculated $P_d$ will vary between episodes. However, the harm incurred by the defense remains relatively constant throughout. These findings can be compared with surveys of repertoires of immune receptors~\cite{Mayer_organized}.

We derived the above filter for a stationary $Q_a$. If the attacker distribution is non-stationary and evolves with time, we can still use the same expressions to estimate $\hat{Q}_a(0)$. This will be sub-optimal but if the timescale of the evolution of $Q_a$ is much slower than the growth rates $\nu_a$ and $\nu'_a$ (which determine how quickly the defenders interact and thereby recognize the attackers), then we can expect the estimate $\hat{Q}_a(t)$ to converge faster than the rate of change of $Q_a(t)$. We will tacitly make this assumption.

\cref{fig:kf_nonstationary} discusses simulation experiments with a non-stationary $Q_a$ with the same setup as that of~\cref{fig:kf_stationary}. We shift the attacker distribution as $Q_{a+k} = Q_a$, i.e., after the $k^{\text{th}}$ episode, the probability of observing attacker $a+k$ is $Q_a$. We can implement this case easily by noticing that the interval [0,1] is isomorphic to [0, 2$\pi$]. This experiment shows how cross-reactivity allows the defenders to both track and counter different types of attacker distributions even if the estimation is not perfect in capturing the large spikes in $Q_a$. The broad trends are similar to those of~\cref{fig:kf_stationary}. But it is interesting to note that the variance of the harm is much smaller in this case than in~\cref{fig:kf_stationary} (top right); this is perhaps because even if the estimate $\hat Q_a(t)$ and the corresponding $P_d^*(\hat Q_a(t))$ are inaccurate, the true attacker distribution changes in the next episode. This suggests that even for non-stationary problems, it is possible to achieve near-optimal harm; cross-reactivity is the key ingredient of the model that makes this possible.

% If the shape space consists of Euclidean locations of the agents, this models mobile attackers.

\begin{figure}
    \centering
    \includegraphics[width=0.49\linewidth]{c3-wd}
    \includegraphics[width=0.49\linewidth]{c3-harms}
    \includegraphics[width=0.49\linewidth]{c3-qa}
    \includegraphics[width=0.49\linewidth]{c3-pd}
    \caption{Estimating an unknown and changing attacker distribution.
    \textbf{Top:} Even when the attacker distribution is changing with time, the filter can track this distribution (the error is slightly higher than the one in~\cref{fig:kf_stationary} top left), and both the defender distribution and the harm incurred are close to their optimal values at the end of the experiment. \textbf{Bottom:} The estimate $\hat Q_a$ now matches the diversity of the true attacker distribution (bottom left) but does not estimate the probabilities of the spikes as accurately. This causes the estimated $P_d^*(\hat Q_a(t))$ to be slightly different than the true $P_d^*(Q_a(t))$ (bottom right).
    }
    \label{fig:kf_nonstationary}
\end{figure}

% From the \textbf{top} plots from of~\cref{fig:kf_nonstationary}, 
% even if the estimation scheme is designed for a stationary $Q_a$, it can track an evolving attacker distribution (left). The initial ($k=0$, blue) and final ($k=300$, orange) attacker distributions $Q_a$ for coefficient of variation $\k=1$ and the final estimation $\hat{Q}_a$ (green) at $k=300$ (right). This shows that it is easier to estimate an evolving attacker distribution with a smaller $\k$.

% \textbf{Middle ($\k=1$) and Bottom ($\k=3$):} We show the final $Q_a$ (blue, right plots) and the estimated $P_d^*(\hat{Q}_a)$ (orange, right plots) for two situations, $\k=1$ (middle) and $\k=3$ (bottom).
% In both cases, the peaks of the the estimated $P_d^*$ track the peaks of $Q_a$. The empirical harm incurred in this experiment (left, orange) converges to the analytical harm (left, green) and is close to optimal harm (left, blue) which is calculated using the true $Q_a$ at each time step.
% The superior tracking for $\k=1$ leads to lower variance in the empirical harm (middle left, orange) and a more biased $P_d^*$ (middle right, orange) that is catered to the final $Q_a(\k=1)$. 
% In contrast, a poorer estimate of $\hat{Q}_a(\k=3)$ (top left, orange) leads to a larger variance in the empirical harm (bottom left, orange). Note how the attacker distribution (blue, middle-bottom right) has more spikes for a larger $\k$. This experiment shows how cross-reactivity allows the defenders to both track and counter different types of attacker distributions.





==> limits.tex <==
% !TEX root = ./root.tex

\section{Limited number of defenders in the repertoire}
\label{s:limits}

The analytical harm in~\cref{eq:Fbar*} is a population-level estimate, i.e., it is valid for an infinite number of attackers and defenders. We will next study the problem when the number of attackers and defenders is finite with the goal of understanding the regime under which this population-level model holds.

Each attacker, out of $N_a$ possible attackers of type $a$, interacts with each defender, out of $N_d$ defenders of type $d$, at each iteration. A recognition event occurs with cross-reactivity probability $f_{d,a}$ and if none of the defenders recognize the attacker, then 1 unit of harm is incurred from each attacker. If one of these interactions is successful, then we set number of attackers of that type to zero. \cref{fig:limits} (left) shows the empirical and analytical harm (calculated using~\cref{eq:Fbar*}) when $\sum_a N_a = \sum_d N_d$, i.e., when the number of attackers is equal to the number of defenders (they are distributed according to their irrespective distributions $Q_a$ and $P_d$). Empirical harm has a larger variance when the number of agents is small, but it is remarkable that our model allows us to estimate this variance accurately. In~\cref{fig:limits} (right), we sweep over both the number of attackers $\sum_d N_a$ and the number of defenders $\sum_d N_d$. We find that, roughly, when the number of attackers $N_a/3 \gtrsim N_d$, the empirical harm is much larger than the analytical harm and the population-level model breaks down.
\todo{there was a comment on why n/3}
%
% As we would expect, the variance of the empirical harm is influenced by the number of defenders and when the number of defenders falls below two times the number of attackers, the variance blows up and we have an empirical harm that exceeds two times the analytical harm.
\begin{figure}[htpb]
    \centering
    \includegraphics[width=0.44\linewidth]{limits_same}%
    \includegraphics[width=0.54\linewidth]{limits_diff}
    \caption{Influence of a limited number of agents on the theory.
    %
    \textbf{Left:} For a fixed $Q_a$ and the corresponding $P_d^*$, we estimate the empirical harm across 100 independent runs for the number of agents $\sum_a N_a = \sum_d N_d \in [1, 1000]$. While the mean empirical harm is close to the analytical harm, the variance of the empirical harm decreases as we increase the number of agents.
    %
    \textbf{Right:} We next sweep both number of attackers $\sum_a N_a$ and the number of defenders $\sum_a N_d$. The analytical harm $\approx 7.113$ for this $Q_a$ and its $P_d^*$; the empirical harm is close to this, roughly up to $\sum_a N_a/3 \gtrsim \sum_d N_d$.
    }
    \label{fig:limits}
\end{figure}

==> mobile.tex <==
% !TEX root = ./root.tex

\section{Modeling mobile defenders}
\label{s:mobile_defenders}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{mobile_def}
    \includegraphics[width=0.49\linewidth]{case5_pd}
    \includegraphics[width=0.49\linewidth]{case5_harm}
    \caption{\textbf{Mobile defenders.}
    \textbf{Top:} Attackers (blue dots) spawn at location $(a, 1)$ with $a \sim Q_a$ and move with constant speed towards the perimeter ($y=0$). For each attacker, a defender (orange dot) spawns at initial state $(d(0), 0)$ with $d(0) \sim P_{d,u}^*$. At every step (indicated by progression of the blue dots, light to dark), defenders move along the perimeter towards their closest attacker with a speed $u$. Interaction between defender and attacker results in a recognition event if they are close ($|d(T)-a|<\e$) at $T=1$.\\[0.25em]
    \textbf{Bottom Left:} For a simple attacker distribution $Q_a$ (blue) with $\s_Q = 0.1$, we show $P_{d,u}^*$ for different speeds $u$ and $\s = 0.01$. As discussed in \cref{s:properties}, when the defender cross-reactivity bandwidth $\s_P=\s$ (or $\s_P=\s u$ for mobile defenders) is less than a threshold $\s_Q \sqrt{1+\a}$, the optimal defender distribution is a Gaussian, otherwise it is a Dirac delta at the mean of the attacker distribution $Q_a$. For $\a = 1$ here, for speeds $u < 14$, the defender distribution is Gaussian, for higher speeds it is a Dirac delta distribution (purple).\\[0.25em]
    \textbf{Bottom Right:} As the speed of defenders increases, we see two regimes for the tradeoff between diversity of defenders and the harm incurred by the defense. For small speeds, $u < 14$, while the shape of the distribution is still close to that of a Gaussian, the diversity of defenders starts reducing because the optimal defense need not maintain too many diverse defender types; the harm remains constant. At higher speeds, the diversity of the defenders reaches a minimum and stays constant while the harm (multiplied by a factor $(\s/\s_Q)^\a$ which ensures that we measure harm at constant recognition probability) increases by a small amount. The expression for the optimal defender distribution can be obtained as discussed in the Appendix; also see (D32)~\cite{Mayer_organized}.
    %
    This implies that \emph{for a fixed recognition probability}, the optimal distribution $P_{d,u}^*$ reduces the number of different types of defenders if they have high mobility due to their larger cross-reactivity, at the cost of incurring a slightly higher harm.
    %Such trade-offs can be used as guiding principles for designing the composition of heterogeneous multi-agent systems.
    }
    \label{fig:mobile_defenders}
\end{figure}

We now formulate the problem where defenders can move to different parts of a Euclidean state-space to intercept attackers. Again the coordinates $a, d \in \reals$ are in Euclidean space. For the perimeter-defense setup, defenders \emph{begin} at location $d$ and can move on the real line with a speed $u$. Attackers arrive at a location $a$. Only the relative speed of the attackers and defenders matters, so we can set the speed of the attackers to be 1. Our key idea is to model the movement of the defenders using the cross-reactivity $f_{d,a,u}$. Consider the scenario where the intruder enters the field of view of the sensors of the defenders when it is 1 unit away from the perimeter. We set
\beq{
    f_{d,a,u} \propto e^{- (d-a)^2/(2 u^2 \s^2)}
    \label{eq:fdau}
}
If $u \ll (d-a)/(2 \s)$, then the probability of interception is small and harm occurs. Our goal is to design the optimal distribution for the defenders $P_{d,u}^*$ that minimizes the harm caused by the attackers who cannot be intercepted. This setup can be solved using the same problem formulation as that of~\cref{s:problem} now by setting
\(
    \Tilde{P_a} = \sum_{d,u} f_{d,a,u} P_{d,u}.
\)
\cref{fig:mobile_defenders} discusses simulation experiments with mobile defenders.

% \begin{figure} [htpb]
%     \centering
%     \includegraphics[width=\linewidth]{c5b1-harms}
%     \includegraphics[width=\linewidth]{case5b1}
%     \caption{Moving defenders and Optimization. maybe i should cut part of the y axis so that we can see the rest of the graph better since its fitting the spike in the beginning}
%     \label{fig:case5b1-harms}
% \end{figure}

==> presentation.tex <==
\section{presentation}
\label{presentation}

\beq{
    \aed{
    \min_{P_d} \quad & \sum_a Q_a \frac{\Gamma(1+\alpha)}{(\sum_d f_{d,a}P_d)^{\a}}\\
    \text{such that}\quad  & P_d \geq 0 \text{ and } \sum_d P_d = 1
    }
    \label{eq:numerical_harm}
}

\\
$\hat{Q}_a(t) = m_a(t)/ \sum_a m_a(t)$
\\
$[-\D, 0, \D] \ni \bar u \sim \pi_{\theta}(d, \hat Q_a)$
\\
$r = - \sum_a \dot m_a(t)$
\\

 Suppose the sensing capability degrades with distance $\norm{q-p}^2$.
 
 The locations of the $n$ sensors $P=(p_1,\dots, p_n)$ can be chosen to maximize 
 
 $\sum_{i=1}^n\int_{V_i}\norm{q-p_i}^2\phi(q)dq$ 
 
 where $V_i = \{ q\in Q \mid \norm{q-p_i} \leq \norm{q-p_j}, \forall j \neq i \}$ is the Voronoi cell.

==> reviews.tex <==
% !TEX root = ./root.tex

\section*{Reviews}
Main point is that our defenders interact with attacker probabilistically and not at every time step, therefore they are sampled based on interactions and our model reflects as such. The model assumes we have an infinite number of defenders and it provides the worst case scenario in a stochastically interacting environment we want to find defender types that maximize the rate of interaction. As such, the model places emphasis in areas or types in the shape space such that the likelihood of interaction is high. Overall it would like the probability of harm from each type of attackers to be uniform so that no single attacker type will cause extreme harm or in other words never be interacted with. If an attacker is sampled from Poisson that means it has interacted with a defender sampled from $P_d$

We are focused on different problem than coverage control where the problem lies in coverage over types. In a 2D space in which attackers exist, the model calculates the percentage or probability that the type of defender is needed in minimize the harm against the given attacking distribution. More defenders simply allow the time to interaction for all attackers to shrink. 
In comparison to coverage control where agents occupy a voronoi cell that does not overlap with its teammates, the model looks to saturate the probability of interaction with the types of attackers in the environment. We see this with competetive dynamics in which defenders spawn and die based on the availability of the attackers. When that function is saturated, defenders spawn in other parts of the state space such that they increase they probability of interaction. 

In the perimeter defense game, if attackers exist, they are interacting with defenders, i.e. there is no poission sample with $\lambda_a(t)$ which defines if they have interacted or not. Next, in the model, we would randomly sample from $P_d$ and call that pair an interaction. Since defenders exist, and have some euclidean space they exist in, a naive allocation can be used to interact with the determinstically existing attackers. Any allocation strategy would improve the harm calculated from the model.  The defenders can then capture via gaussian capture or point wise position capture where they would have to move based on the allocation.

Some questions to answer
\begin{itemize}
    \item emphasize heterogeneity
    \item why is the cross reactivity gaussian?
    \item is it reliable to use probabilistic models to model the interaction between attackers and defenders? I imagine yes, its a game scenario where sides send troops out, they make a determin
    \item lack of theoretical analysis on the performance of the proposed model and defending policy
    \item a brief description of the shape space is needed. we define the shape space as $x \in [0,1]$ where we discretize $x$ to be the types of agents (generally 200). As seen in figure 1, types can refer abstractly to the capabilities of the agents or locations measures in the euclidean space.
    \item why is the diversity of the defense defined by th L0 norm? The metric can be 30 or 50 depending on the discritization of the space. in this case there are 50 types. 30 would be there are 30/50 discrete types. This is different than the total number of attackers. In each iteration we sample 100 attackers from $P_d$ that might have 30 different types. $N_a$ and $N_d$ 
    \item fig 3 what is the meaning of the green curve? the green curve shows the proabability of harm coming that that discrete type of attacker. As you can see it is close to uniform except in the case where the types where there are the largest probability of attacker. Based on euqation 3 harm is a real number and in this plot we do not sum over the types and we normalize to 1 to be a probability.
    \item fig 3 right even though the defenders have different cross reactivities, they all have a chance to interact with each type of attacker and are not limited to their third of the domain. This plot shows that if an attacker happens to interact with a defender of large cross-reactivity it is more likely to be recognized and therefore the harm to the repertoire by these types of attackers is minimal.
    \item fig 4 what is the values of the bandwidth? it is $\sigma= 0.5$ where there are 200 types (discrete bins). why is the difference between emprical and analytical small when there are at most 3 times more attackers than defenders. This is do to availability of the defenders. the analytical result assumes we have infinite att and def. Experimentally we see that if these assumptions do not hold the analytical result stays true until there are more than 3 times the def numbers. This is due to assignment, where the interactions are 1 to 1.
    \item no result on how $N_a$ and $N_d$ vary over time. $N_d$ stays infinite in sim. $N_a$ decreases over time until all of them have been recognized (we can see this with fat and lat).
\end{itemize}

==> v0/basic.tex <==
% !TEX root = ./root.tex

\section{Optimal defender distribution is supported on a discrete set}
\label{s:properties}

Our cross-reactivity term models the fact that in biology, a given receptor can bind to different pathogens to varying degrees: a non-zero bandwidth $\s$ allows the organism to reduce the number of different types of defenders that it needs to maintain to tackle typical attackers. For a Gaussian $Q_a \propto e^{-a^2/(2 \s_Q^2)}$,~\cite{Mayer_organized} shows that when the cross-reactivity bandwidth $\s$ is smaller than a threshold $\s_Q \sqrt{1+\a}$, the optimal defender distribution is also Gaussian
\[
    P_d^* \propto e^{-\f{d^2}{2 ( (1 + \a)\s_Q^2 -\s^2 )}}.
\]
Note that the variance is negative if $\s/\s_Q > \sqrt{1+\a}$. So if the bandwidth is above this threshold, the optimal defense is a Dirac delta at the origin. This shows that cross-reactivity allows concentrated distributions and reduces the need to maintain a diverse number of defenders. We can also show this mathematically where we can turn the variational problem in~\cref{eq:harm} into a standard optimization problem by assuming a parametric form for the defender distribution $P_d = e^{-d^2/(2 \s_P^2)}$ (by symmetry it has to be centered at $d=0$). For a Gaussian $Q_a$, we can now minimize the harm in~\cref{eq:harm}, to see that the solution has $\s_P = 0$.

Such discreteness is also seen in many other problems, e.g., capacity of a Gaussian channel under an amplitude constraint~\cite{smith1971information} and representations in the brain~\cite{laughlin1981simple}. A somewhat related phenomenon can also be found in the statistics literature which studies priors that are supported over a discrete set~\cite{berger2009formal}. In intuitive terms, a discrete prior (or a discrete defender distribution) allows capturing large parts of the data space (or the attacker distribution) with few resources (models or receptors). These ideas have been studied in information theory~\cite{mattingly2018maximizing} and have also been used to build new methods to learn from unlabeled data in the machine learning literature~\cite{gao2022deep}. In our case, the optimal defender distribution $P_d^*$ also puts its probability mass on diverse types of defenders to best tackle the attackers using the cross-reactivity. Larger the cross-reactivity bandwidth $\s$, more the spacing in between the atoms of $P_d^*$. Although, we have argued discreteness in the setting when $Q_a$ is Gaussian, this result is expected to hold in general; see the numerical simulation in~\cref{fig:case0}.

\subsection{A toy perimeter-defense problem with immobile attackers and defenders}

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{case0}\\
    \includegraphics[width=0.9\linewidth]{case0tv}
    \caption{\textbf{Top:} Defenders protect a perimeter $[0,1]$ from attackers with distribution $Q_a$ supported on $[0,1]$. Probabilities $Q_a$ are drawn from a log-normal distribution with coefficient of variation $\kappa^2 = \exp(\s_Q^2)-1$ and normalized (blue). The optimal defender distribution $P_d^*$ (orange) is found by optimizing~\cref{eq:harm}. A cross-reactivity kernel $f_{d,a}$ of bandwidth $\s = 0.05$ leads to a discrete distribution that covers the state space. In green, we show the harm $\Bar{F}_a$ caused by attackers at different locations $a$ weighted by their probability $Q_a$. This harm is relatively constant in spite of a discrete distribution $P_d^*$ because of the cross-reactivity kernel $f_{d,a}$ with a non-zero bandwidth $\s$. The number of spikes in $P_d^*$ will reduce for a larger $\s$ and although the overall harm  $\sum_a Q_a \Bar{F}_a $ will increase, the harm by every attacker $\Bar{F}_a$ will be relatively constant.\\[0.25em]
    %
    \textbf{Bottom:} The harm incurred using a non-optimal $P_d$ is close to that of the harm of $P_d^*$ in~\cref{fig:case0} even for large differences, as measured in the total variation norm ($\f{1}{2}\norm{P_d-P_d^*}_1$). To obtain this plot,  we sampled 1000 different $P_d$s (by perturbing the optimal $P_d^*$ using log-normal noise) and computed the empirical and analytical harm against a fixed $Q_a$. This experiment also indicates that the empirical harm calculated using our experiments using~\cref{eq:Fbar} is close to the analytical harm~\cref{eq:Fbar*} for a broad regime.
    }
    \label{fig:case0}
\end{figure}

We first discuss how cross-reactivity helps tackle heterogeneity using a toy problem where neither defenders nor attackers can ``move''. Imagine that a fixed number of attackers spawn according to the attacker distribution $Q_a$ and move with constant velocity towards a perimeter. Similarly, a fixed number of defenders spawn on the perimeter according to the defender distribution $P_d$. For a 1-dimensional perimeter defense problem, let us have the defenders be on the real line and they can only interact with attackers who seek to penetrate the line; see~\cref{fig:case0}. The shape space here is the Euclidean location of the attackers and defenders. Defenders that are close to attackers are able to interact with the attacker with a higher probability and if the interaction succeeds, they can prevent harm. On the other hand, defenders that are very far away from the attacker have a small probability of successfully interacting with the attackers and are thus unable to stop the harm. The goal of the defense team is to place defenders along the perimeter and minimize the number of attackers that successfully penetrate the perimeter. This setting can be exactly captured by our model; the optimal defender distribution is shown in~\cref{fig:case0}.

==> v0/competition.tex <==
% !TEX root = ./root.tex

\section{Decentralized control: Competition between defenders leads to optimal resource allocation}
\label{s:competition}

The optimal defender distributions $P_d^*$ or $P_{d,u}^*$ were calculated in a centralized fashion. In this section, we discuss how we can achieve optimal harm even if the control policy for the defenders, namely $P_d^*$ is calculated in a decentralized fashion. The key idea is to exploit cross-reactivity between the defenders, i.e., the fact that multiple defenders can tackle the same attacker and set up competition among the defenders to earn the reward of successfully recognizing an attacker. Biology is similar, receptors that successfully recognize antigens proliferate at the cost of other receptors~\cite{DEBOER1994375}.

Let the number of defenders of a particular type be $N_d$. We can set
\beq{
    \dv{N_d}{t} = N_d \sbr{\sum_a Q_a \varphi \rbr{\sum_{d'} N_{d'} f_{d',a}} f_{d,a} - c}.
    \label{eq:competition}
}
Here, the constant $c$ is the rate at which defenders $d$ are decommissioned (the death rate in biology). In the first term, the total interaction of defender $d$ with different attackers $\sum_a Q_a f_{d,a}$ is weighted by some function $\varphi(\cdot)$ which is a decreasing function of its argument. The quantity $\sum_{d'} N_{d'} f_{d',a}$ determines how many other defenders can tackle $a$. If this is large, then the incremental utility of having the specific defender $d$ diminishes, and therefore its growth rate $\dot{N}_d$ should be smaller. We will see in experiments that the harm caused by this decentralized dynamics converges to the optimal harm obtained from a centralized computation of $P_d^*$. We can also use the estimated attacker distribution $\hat{Q}_a$ in place of the true distribution $Q_a$ in~\cref{eq:competition} in situations where it is unknown to the defenders.

\cref{fig:competition_stationary} shows an experiment with decentralized control when the attacker distribution $Q_a$ is stationary while~\cref{fig:competition_nonstationary} shows a similar result when defenders estimate an evolving attacker distribution using the filter in~\cref{s:evolving}. We have also obtained similar results for the case when defenders move and tackle a stationary attacker distribution (like that of~\cref{s:mobile_defenders}).

\begin{figure}[htpb]
    \centering
    % \includegraphics[width=\linewidth]{c2b-harms}
    % \includegraphics[width=\linewidth]{case2b}
    % \includegraphics[width=0.49\linewidth]{c2b-tv}
    \includegraphics[width=0.49\linewidth]{c2b-harms}
    % \includegraphics[width=0.49\linewidth]{c2b-qa}
    \includegraphics[width=0.49\linewidth]{c2b-pd}
    \caption{\textbf{Convergence to near-optimal harm using decentralized control.}
    For the same setting as that of~\cref{fig:kf_stationary}, we run the dynamics in~\cref{eq:competition} using the estimate $\hat{Q}_a(t)$ calculated using the Kalman filter to induce the optimal defender distribution $P_d^*(t)$ (instead of calculating it by minimizing the harm in~\cref{eq:harm} as done in~\cref{fig:kf_stationary}). The harm in this case is slightly lower than that in~\cref{fig:kf_stationary}, perhaps because of the transient dynamics in~\cref{eq:competition} which does not lead to $P_d^*$ immediately but models the growth of defenders over time. We run the population dynamics for $10^6$ iterations within each episode to obtain $P_d^*$. The defender distribution (orange, right) is again close to the optimal distribution $P_d^*$ for $Q_a$ but note that it is a bit smoother (and therefore sub-optimal). We know from~\cref{fig:mobile_defenders} that there is a tradeoff between the diversity of the defender types (many types for a smooth distribution to few types for a spiked distribution) and harm (lower harm for the smooth distribution and higher harm for same recognition probability for the latter).
    }
    \label{fig:competition_stationary}
\end{figure}

% \begin{figure} [htpb]
%     \centering
%     \includegraphics[width=0.75\linewidth]{case0_dec}
%     \caption{Competitive dynamics encourage defenders to self-organize into a state that encourages maximum interaction and in turn minimal harm.}
%     \label{fig:case0-dec}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.4\linewidth]{case3b-tv}
    \includegraphics[width=0.4\linewidth]{case3b-initfinalqa}\vspace*{-0.5em}
    \includegraphics[width=0.4\linewidth]{c3b-harms}
    \includegraphics[width=0.4\linewidth]{case3b-pdk1}\vspace*{-0.5em}
    \includegraphics[width=0.4\linewidth]{c3b_kappa3-harms}
    \includegraphics[width=0.4\linewidth]{case3b-pdk3}
    \caption{
    \textbf{Convergence to near-optimal harm using decentralized control for the case when the attacker distribution evolves across episodes.}
    For the same setting as that of~\cref{fig:kf_nonstationary}, i.e., when the attacker distribution shifts as $Q_{a+k} = Q_a$, we implemented the decentralized control dynamics using the estimate $\hat{Q}_a$ obtained by the defenders. We have implemented a centralized estimation problem in this case, i.e., all defenders share information of their interactions with each other and thereby maintain a single estimate $\hat{Q}_a$.\\[0.25em]
    \textbf{Top:} We show $Q_a$ with coefficient of variation $\k=3$ for the initial ($k=0$) and final ($k=300$) attacker distributions and the final estimation $\hat{Q}_a$ at $k=300$ (right). Like~\cref{fig:kf_nonstationary}, the TV plot (left) shows that estimation of $Q_a$ is easier for a smaller $\k$.\\[0.25em]
    \textbf{Middle ($\k=1$) and Bottom ($\k=3$):} Like~\cref{fig:competition_stationary}, the decentralized formulation gives rise to smooth defender distributions (orange, right). In the middle row, the distribution $Q_a$ is less spiked and therefore the decentralized defender distribution is more spiked (and closer to the optimal one, as indicated by the empirical harm in orange vs. analytical harm in blue in the middle left plot). In the bottom row, the attacker distribution $Q_a$ is more spiked which makes it more difficult to be estimated by the filter. Consequently, the defender population induced by the decentralized dynamics is also sub-optimal (orange in bottom right is farther away from optimal, as indicated by the empirical harm in orange being farther away from the optimal harm in blue in the bottom left plot). The empirical harm for $\k=3$ again has a higher variance than that of the middle row. This experiment indicates that the decentralized population dynamics in~\cref{eq:competition} is capable of both tracking and countering an evolving attacker distribution.
    }
    \label{fig:competition_nonstationary}
\end{figure}

==> v0/intro.tex <==
% !TEX root = ./main.tex

\section{Introduction}
\label{s:intro}

\begin{wrapfigure}{r}{0.49\linewidth}
\centering
\includegraphics[width=\linewidth]{figures/figure1.pdf}
\end{wrapfigure}
Consider two teams, denoted by ``defenders'' (orange) and ``attackers'' (blue), each with a heterogeneous group of agents that have different capabilities, say offensive or defensive skills, or mobility. The defenders seek to protect an area against the attacking team which tries to penetrate this defense. The goal of this paper is to understand control policies for the defenders that take into account the heterogeneous nature of this problem.

We draw inspiration from the adaptive immune system which faces a similar problem while protecting an organism from pathogens~\cite{Mayer_organized}. Some pathogens are persistent but benign (e.g, common cold) and others are rare but dangerous (e.g., HIV). There is a vast number of other pathogens on this spectrum. Tackling every pathogen optimally requires a specialized receptor (these are proteins expressed by lymphocytes whose molecules bind to the molecular constitution of pathogens). It would intuitively seem that the distribution of such receptors should be identical to the distribution of pathogens in the environment. But such a diverse repertoire would come at a large metabolic cost of maintaining all these receptors. The immune system builds a rather non-intuitive repertoire: it devotes relatively more resources to fighting pathogens that cause large harm even if they are rare and relatively fewer resources to pathogens which cause less harm even if they are encountered frequently. Such a composition seems counter-intuitive. There are two key reasons which lead to its emergence. First, a constraint on the metabolic energy spent on maintaining a large receptor repertoire limits the total number of diverse receptors. And second, there exist specialized receptors that detect and tackle a specific pathogen with high probability but these receptors can also respond to other similar pathogens with a smaller probability and thereby reduce the overall harm to the organism. This paper embodies these ideas into control policies for the defender team.

% \begin{figure}[htpb]
%     \centering
%     \includegraphics[width=0.75\linewidth]{figures/figure1.pdf}
%     \caption{Consider the perimeter-defense game in which a team of attackers (blue) attempt to penetrate a perimeter guarded by defenders (orange). Attackers and defenders spawn according to their respective distributions.}
%     % In this paper, we model the how a defense would organize itself under the constraints that (i) no single defender can defend against every type of attacker and (ii) the defense has limited resources and must decide on how to best allocate and organize its team.}
%     \label{fig:intro}
% \end{figure}

\subsection{Contributions}

% We use a perimeter-defense setting to study (i) estimating the attacker distribution leads to near-optimal harm (as if the attacker distribution was known in advance), (ii) the performance when the attacker distribution shifts in time, and (iii) how competition between defenders leads to near-optimal harm.

\textbf{We use a theoretical model of the immune system~\cite{Mayer_organized} to understand perimeter-defense problems with heterogeneous teams of multiple agents.} The defender team seeks to select the appropriate type of agents and an appropriate number of them to minimize the harm caused by a heterogeneous attacker team.  We seek to understand two situations: (i) when no single defender can defend against every type of attacker, and (ii) when defenders have limited resources that they should devote optimally to tackle the attackers.

\textbf{We develop a technique to estimate an unknown attacker distribution.} Defenders may not always have full knowledge of the attacker distribution. In this situation, it may be possible to use the information from defender-attacker encounters in a Bayesian filter to estimate the attacker distribution and adapt the defender distribution accordingly. We consider two situations: (i) when the attacker distribution is stationary and does not change over time, and (ii) when it evolves over time.

\textbf{We show that the defender team can achieve near-optimal harm using a decentralized approach.} Centralized computation may seem necessary to select the optimal defender distribution because both local and global structure of the attacker distribution determines it. We study decentralized dynamics where competition between defenders for successful interaction with attackers acts as a reward to encourage the congregation of specific defender types. We show how such local computation leads to near-optimal defender distributions, both when the attacker distribution is stationary, and when it evolves over time. We also study the ``centralized estimation and decentralized control'' setting where information obtained from individual interactions with the attackers is shared with all the defenders but the competitive dynamics of the defenders is decentralized.

\subsection{Organization} We first formulate the model in~\cref{s:problem}. We investigate the model under different scenarios using theory and simulation experiments in~\cref{s:properties,s:mobile_defenders,s:evolving,s:competition}. We discuss related work in~\cref{s:related_work}.

==> v0/kf.tex <==
% !TEX root = ./root.tex

\section{Estimating an unknown attacker distribution}
\label{s:evolving}

Next we are interested in understanding settings where the attacker distribution $Q_a$ is not known to the defenders and it may change over time. The attacker distribution can change in two ways, either there are different types of attackers that arrive as time progresses, or the attackers move in the state-space. We will discuss how to estimate $Q_a(t)$ and use this estimate to calculate a new optimal distribution for the defenders $P_d^*(t)$ at each time step. Interactions, both successful recognition events or unsuccessful ones, give observations of the attacker types $a$ and thereby $Q_a(t)$.

\begin{figure}[!htpb]
    \centering
    % \includegraphics[width=\linewidth]{c2-harms}
    % \includegraphics[width=\linewidth]{case2}
    \includegraphics[width=0.49\linewidth]{c2-tv}
    \includegraphics[width=0.49\linewidth]{c2-harms}
    \includegraphics[width=0.49\linewidth]{c2-qa}
    \includegraphics[width=0.49\linewidth]{c2-pd}
    \caption{\textbf{Estimating an unknown and stationary attacker distribution.}
    We initialize $\hat{Q}_a(0)$ to be uniform and set $P_d^*(0)$ using~\cref{eq:harm}. The Kalman filter-based technique in~\cref{s:evolving} is run for 300 episodes. At the beginning of each episode, we sample a new set of attackers from $Q_a$ and within every episode $0 \leq t \leq T$, we sample defenders from $P_d^*(t)$ that is calculated on the basis of $\hat{Q}_a(t)$. The episode ends at a random time $T$ when the last attacker is recognized by the defense and total harm of the episode is the harm incurred until all attackers are recognized. The estimate of $\hat{Q}_a$ is initialized to its final value $\hat{Q}_a(T)$ from the previous episode. In other words, defenders get multiple opportunities to estimate the attacker distribution but \emph{attacker types} can be different across episodes.\\[0.25em]
    %
    \textbf{Top:}
    The total-variation distance between the true $Q_a$ and the estimated $\hat{Q}_a$ decreases with the number of episodes (left). Remarkably, harm incurred by the defenders using the estimated $\hat{Q}_a$ (green,~\cref{eq:Fbar*}) converges to the optimal harm as if $Q_a$ was known perfectly (blue) as the defenders see more episodes. The empirical harm (orange,~\cref{eq:Fbar}) is also close to the analytical harm (green). The large spikes in the right plot are due to noisy observations resulting from suboptimal defender distributions which further result in an inaccurate estimate of $\hat{Q}_a$. But once $\hat{Q}_a$ stabilizes (around 100 episodes), the harm in subsequent episodes is at most twice the optimal.\\[0.25em]
    \textbf{Bottom:}
    We show the final $\hat{Q}_a$ estimated at the end of 300 episodes (orange) against the actual $Q_a$ (blue) in the left plot. The corresponding defender distributions $P_d^*(\hat{Q}_a)$ (orange) and $P_d^*(Q_a)$ (blue) are shown on the right. Note that even if the estimation procedure does not recover the exact $Q_a$, the defender distribution for the estimated $\hat{Q}_a$ is very similar to the defender distribution for the true $Q_a$, as is the harm in the top right plot. This indicates that in these highly stochastic problems with multiple agents (we have 1000 attackers and 1000 defenders) we can still meaningfully counter an unknown attacker distribution and obtain a defender distribution that incurs the optimal harm.
    }
    \label{fig:kf_stationary}
\end{figure}

Our model for how attackers proliferate enables us to estimate their distribution as follows. Let us first assume that $Q_a$ is unknown to the defenders but it is stationary, i.e., it does not change with time. From~\cref{s:problem}, the expected number of attackers is $m_a(t)$ and it grows as $m_a(t) = m_a(0) e^{\nu_a t}$. Since we have $m_a(0) = 1$ for attackers $a$ that were sampled from $Q_a$, if we can estimate $\hat{m}_a(0)$ then we can think of the attackers corresponding to it as sampled from $Q_a$ and therefore obtain an estimate of $Q_a$.

Let us arrange all the attackers into a large vector $x(t) \in \reals^{m_a(t)}$ which will be the state of the filter. We will assume that $x_i \sim N(\mu_i, \s_i)$ for $i \leq m_a(t)$; observations $y_i = c x_i + \xi$ where $c$ is a Boolean that indicates if this specific attacker interacted with the defenders; $\xi \sim N(0, \s_\xi^2)$ is Gaussian noise. We can update $\mu_i^+ = \mu_i + k (y_i - c \mu_i)$ and $(\s_i^+)^2 = (1 - k c) \s_i^2$ using the Kalman gain $k = \s_i^2 c/(c^2 \s_i^2 + \s_\xi^2)$. The growth rate is estimated as $\hat{\nu}_i = \log (\mu_i^+/\mu_i)$. Since there are multiple attackers for each type, we average the estimates as
\[
        \hat{\mu}_a(t) = \f{\sum_{i=1}^{m_a(t)} \ind{\text{type }(x_i) = a} \mu_i}{\sum_{i=1}^{m_a(t)} \ind{\text{type }(x_i) = a}},
\]
and similarly for $\hat{\nu}_a$ to get $\hat{Q}_a(t) = \hat{\mu}_a e^{- \hat{\nu}_a t}$. Let us emphasize that the number of attackers $m_a(t)$ (and therefore the dimensionality of the state $x$ of the filter) growing with time is not an issue in the implementation. As discussed, the filter runs independently for each attacker (and therefore each attacker type) but is easy to incorporate a known model of the correlations between the growth rates $\nu_a$ of different attacker types. Given the estimate of $\hat{Q}_a(t)$, we recalculate the optimal defender distribution $P_d^*(t)$ by minimizing~\cref{eq:harm} at each instant. \cref{fig:kf_stationary} discusses simulation experiments with a stationary $Q_a$.

% In~\cref{fig:case2-harms} (A), we see similarly to~\cref{fig:case1} that the $\text{TV}(Q_a, \hat{Q}_a)$ decreases over time as the estimate $\hat{Q}_a$ get close to the true $Q_a$. Although the estimate is not exact as shown by the curve stabilizing at around 0.4 $\text{TV}(Q_a, \hat{Q}_a)$ but the harm caused to $P_d$ is close the harm caused to $P_d^*$. Why might this be the case?

% It can be seen that due to cross-reactivity, the optimal defender distribution is spiked according to the cross-reactive width, $\sigma$, and uniformly covers the perimeter. This characteristic of the defensive distribution is an important consequence for when we have different samples from the same attacker distribution. Each episode, the defense will observe a slightly different spectrum of attackers because of the stochasticity of observations and the resulting calculated $P_d$ will vary between episodes. However, the harm incurred by the defense remains relatively constant throughout. These findings can be compared with surveys of repertoires of immune receptors~\cite{Mayer_organized}.

The above expressions for $\hat{Q}_a(t)$ are derived for a stationary $Q_a$. If the attacker distribution is non-stationary and evolves with time, then we can still use the same expressions to estimate $\hat{Q}_a(0)$ but doing so will incur errors. But if the timescale of the evolution of $Q_a$ is much slower than the growth rates $\nu_a$ and $\nu'_a$ (which determine how quickly the defenders interact and thereby tackle the attackers), then we can expect the estimate of $\hat{Q}_a(t)$ to converge faster than the evolution of $Q_a(t)$. In this paper, we do not focus on accurately tracking such evolving attacker distributions and instead use this simple trick. \cref{fig:kf_nonstationary} discusses simulation experiments with a non-stationary $Q_a$.

% \begin{figure} [htpb]
%     \centering
%     \includegraphics[width=\linewidth]{case1}
%     \todo[inline]{Chris: this figure seems to be the same as the one in~\cref{fig:kf_stationary}? What is the difference and can we remove it?}
%     \todo[inline]{Pratik: this is the case where we use a uniform dist for Pr to start and only use KF to estimate. it is probably not that important of an experiment}
%     \caption{In (A), the defenders utilize a uniform $P_d$ to recover $Q_a$ using the KF approach. Over episodes of the environment, defender's local observations of the intruders updates the KF and the resulting belief, $\hat{Q}_a$. In (B), we display the total variation, TV($Q_a, \hat{Q}_a$), over episodes to show $\hat{Q}_a$ gets close to the true $Q_a$.}
%     \label{fig:case1}
% \end{figure}

% \begin{figure} [htpb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{c1-TV.png}
%     \caption{Given the setup of Fig.(\cref{fig:case1}), we display the total variation, TV($Q_a, \hat{Q}_a$), decreasing over episodes to show $\hat{Q}_a$ getting close to the true $Q_a$.}
%     \label{fig:case1-TV}
% \end{figure}

\begin{figure}
    \centering
    \includegraphics[width=0.395\linewidth]{case3-tv}
    \includegraphics[width=0.395\linewidth]{case3-initfinalqa}\vspace*{-0.5em}
    \includegraphics[width=0.395\linewidth]{c3-harms}
    \includegraphics[width=0.395\linewidth]{case3-pdk1}\vspace*{-0.5em}
    \includegraphics[width=0.395\linewidth]{c3_kappa3-harms}
    \includegraphics[width=0.395\linewidth]{case3-pdk3}
    \caption{\textbf{Estimating a changing attacker distribution.}
    For the same setting as that of~\cref{fig:kf_stationary}, we run the filter when the attacker distribution shifts as $Q_{a+k} = Q_a$, i.e., after the $k^{\text{th}}$ episode the probability of observing attacker $a+i$ is $Q_a$. The interval $[0,1]$ is set to be isomorphic to $[0, 2\pi]$ in this case by setting $a=0$ and $a=1$ to be the same points. If the shape space consists of Euclidean locations of the agents, this models mobile attackers.\\[0.25em]
    \textbf{Top:} Even if the estimation scheme is designed for a stationary $Q_a$, it can track an evolving attacker distribution (left). The initial ($k=0$, blue) and final ($k=300$, orange) attacker distributions $Q_a$ for coefficient of variation $\k=1$ and the final estimation $\hat{Q}_a$ (green) at $k=300$ (right). This shows that it is easier to estimate an evolving attacker distribution with a smaller $\k$. \\[0.25em]
    \textbf{Middle ($\k=1$) and Bottom ($\k=3$):} We show the final $Q_a$ (blue, right plots) and the estimated $P_d^*(\hat{Q}_a)$ (orange, right plots) for two situations, $\k=1$ (middle) and $\k=3$ (bottom).
    In both cases, the peaks of the the estimated $P_d^*$ track the peaks of $Q_a$. The empirical harm incurred in this experiment (left, orange) converges to the analytical harm (left, green) and is close to optimal harm (left, blue) which is calculated using the true $Q_a$ at each time step.
    The superior tracking for $\k=1$ leads to lower variance in the empirical harm (middle left, orange) and a more biased $P_d^*$ (middle right, orange) that is catered to the final $Q_a(\k=1)$. In contrast, a poorer estimate of $\hat{Q}_a(\k=3)$ (top left, orange) leads to a larger variance in the empirical harm (bottom left, orange). Note how the attacker distribution (blue, middle-bottom right) has more spikes for a larger $\k$. This experiment shows how cross-reactivity allows the defenders to both track and counter different types of attacker distributions.
    }
    \label{fig:kf_nonstationary}
\end{figure}


==> v0/mobile.tex <==
% !TEX root = ./root.tex

\section{Modeling mobile defenders}
\label{s:mobile_defenders}

\begin{figure}
    \centering
    \includegraphics[width=0.9\linewidth]{mobile_def}
    \includegraphics[width=0.49\linewidth]{case5_pd}
    \includegraphics[width=0.49\linewidth]{case5_harm}
    \caption{\textbf{Mobile defenders.}
    \textbf{Top:} Attackers (blue dots) spawn at location $(a, 1)$ with $a \sim Q_a$ and move with constant speed towards the perimeter ($y=0$). For each attacker, a defender (orange dot) spawns at initial state $(d(0), 0)$ with $d(0) \sim P_{d,u}^*$. At every step (indicated by progression of the blue dots, light to dark), defenders move along the perimeter towards their closest attacker with a speed $u$. Interaction between defender and attacker results in a recognition event if they are close ($|d(T)-a|<\e$) at $T=1$.\\[0.25em]
    \textbf{Bottom Left:} For a simple attacker distribution $Q_a$ (blue) with $\s_Q = 0.1$, we show $P_{d,u}^*$ for different speeds $u$ and $\s = 0.01$. As discussed in \cref{s:properties}, when the defender cross-reactivity bandwidth $\s_P=\s$ (or $\s_P=\s u$ for mobile defenders) is less than a threshold $\s_Q \sqrt{1+\a}$, the optimal defender distribution is a Gaussian, otherwise it is a Dirac delta at the mean of the attacker distribution $Q_a$. For $\a = 1$ here, for speeds $u < 14$, the defender distribution is Gaussian, for higher speeds it is a Dirac delta distribution (purple).\\[0.25em]
    \textbf{Bottom Right:} As the speed of defenders increases, we see two regimes for the tradeoff between diversity of defenders and the harm incurred by the defense. For small speeds, $u < 14$, while the shape of the distribution is still close to that of a Gaussian, the diversity of defenders starts reducing because the optimal defense need not maintain too many diverse defender types; the harm remains constant. At higher speeds, the diversity of the defenders reaches a minimum and stays constant while the harm (multiplied by a factor $(\s/\s_Q)^\a$ which ensures that we measure harm at constant recognition probability) increases by a small amount. The expression for the optimal defender distribution can be obtained as discussed in the Appendix; also see (D32)~\cite{Mayer_organized}.
    %
    This implies that \emph{for a fixed recognition probability}, the optimal distribution $P_{d,u}^*$ reduces the number of different types of defenders if they have high mobility due to their larger cross-reactivity, at the cost of incurring a slightly higher harm.
    %Such trade-offs can be used as guiding principles for designing the composition of heterogeneous multi-agent systems.
    }
    \label{fig:mobile_defenders}
\end{figure}

We now formulate the problem where defenders can move to different parts of a Euclidean state-space to intercept attackers. Again the coordinates $a, d \in \reals$ are in Euclidean space. For the perimeter-defense setup, defenders \emph{begin} at location $d$ and can move on the real line with a speed $u$. Attackers arrive at a location $a$. Only the relative speed of the attackers and defenders matters, so we can set the speed of the attackers to be 1. Our key idea is to model the movement of the defenders using the cross-reactivity $f_{d,a,u}$. Consider the scenario where the intruder enters the field of view of the sensors of the defenders when it is 1 unit away from the perimeter. We set
\beq{
    f_{d,a,u} \propto e^{- (d-a)^2/(2 u^2 \s^2)}
    \label{eq:fdau}
}
If $u \ll (d-a)/(2 \s)$, then the probability of interception is small and harm occurs. Our goal is to design the optimal distribution for the defenders $P_{d,u}^*$ that minimizes the harm caused by the attackers who cannot be intercepted. This setup can be solved using the same problem formulation as that of~\cref{s:problem} now by setting
\(
    \Tilde{P_a} = \sum_{d,u} f_{d,a,u} P_{d,u}.
\)
\cref{fig:mobile_defenders} discusses simulation experiments with mobile defenders.

% \begin{figure} [htpb]
%     \centering
%     \includegraphics[width=\linewidth]{c5b1-harms}
%     \includegraphics[width=\linewidth]{case5b1}
%     \caption{Moving defenders and Optimization. maybe i should cut part of the y axis so that we can see the rest of the graph better since its fitting the spike in the beginning}
%     \label{fig:case5b1-harms}
% \end{figure}

==> v0/problem.tex <==
% !TEX root = ./root.tex

\section{Problem Formulation}
\label{s:problem}

Let $Q_a$ be the probability that denotes the next intrusion will be caused by an attacker of type $a$. Let $P_d$ be the probability of a defender of type $d$ being present. We wish to compute the optimal distribution of the defenders $P_d^*$ that minimizes the harm caused by this intrusion. In biology, attackers $a$ and defenders $d$ interact in an abstract state-space called the shape-space~\cite{PERELSON1979645}.

In this paper, we will be deliberately vague about what the state-space is. For studying steady-state situations when there is a large number of attackers and defenders, we will think of the shape space as the types of agents (a defender of type $d$ interacts with an attacker of type $a$); for studying situations when defenders or attackers are mobile, we will think of the shape space as the Euclidean state-space ($a, d$ are locations of agents).

\paragraph{Interaction between attackers and defenders}
Let us first model the situation when defenders are stationary on/inside the perimeter and get observations from the attackers when both are within a certain distance of each other. We will use a cross-reactivity term $f_{d,a}$ to denote the probability that defender $d$ tackles an attacker $a$ successfully. While the cross-reactivity can be any kernel, we will focus on a Gaussian $f_{d,a} \propto \exp\rbr{-\f{(d-a)^2}{2\s^2}}$ where $\s$ denotes the bandwidth (as mentioned above, $\s$ can refer to the different types of agents, or Euclidean locations). Far away defenders under this kernel have a smaller chance of tackling attackers. The total probability of tackling an attacker $a$ successfully is $\Tilde{P}_a = \sum_d f_{d,a} P_d$.

We can model the interaction between an attacker $a$ and some defender $d$ as a Poisson random variable with rate $\l_a(t)$. Larger the number of attackers, larger the rate of interaction with them; we model this as a rate that increases exponentially with time $\dot{\l}_a(t) = \l_a \nu'_a$ starting from some initial rate $\l_a(0) = 1$ (for sampled $a \sim Q_a$). In biology, this is because the population of pathogens grows. For us it is because the attacker spends more time in the environment. The expected number of interactions of an attacker with some defender is $m_a(t) = \int_0^t \dd{\t} \l_a(\t) \approx \l_a(0) (e^{\nu'_a t - 1})/\nu'_a$.

\paragraph{Harm caused by an attacker}
The number of attackers of a type $a$ denoted by $m_a(t)$ also grows exponentially $\dot{m_a}(t) = m_a \nu_a$ starting from some $m_a(0) = 1$ (for sampled $a \sim Q_a$) if it is not tackled successfully. The exponents $\nu_a$ and $\nu_a'$ may be different because the number of attackers $a$ that cause harm may grow differently than the number of attackers $a$ that can be observed by the defense. Unsuccessful interactions of defenders with attackers cause one unit of harm. For large times $t \approx \log(m_a/\l_a(0))/\nu'_a$, the expected harm caused by an attacker of type $a$ after $m$ unsuccessful interactions is
\beq{
    F_a(m) = F_a(0) \rbr{\f{m}{\l_a(0)}}^{\nu_a/\nu'_a} \propto m^\a;
    \label{eq:fm}
}
where $\a = \nu_a/\nu'_a$. The quantity $F_a(m)$ is polynomial in the number of interactions $m$ in this paper but it can also take other forms, e.g., $F_a(m) = 1 - e^{-\b m}$ would model the situation where the harm plateaus after a large number of interactions. The harm $\Bar{F}_a$ caused by an attacker $a$ is thus the average recognition time
\beq{
    \Bar{F}_a = \Tilde{P}_a \int_0^{\infty} \dd{m} F_a(m) e^{-m \Tilde{P}_a}.
    \label{eq:Fbar}
}
We call this the ``empirical harm'' because we will be able to estimate it using simulations.

\paragraph{Minimizing the harm}
The harm caused by an attacker sampled from $Q_a$ is
\beq{
    \text{Harm}(P_d) = \sum_a Q_a \Bar{F}_a.
    \label{eq:harm}
}
It is a function of the defender distribution $P_d$ and our goal will be to minimize it. When $F_a(m) = m^\a$, the optimization problem can be solved analytically to obtain the mean harm
\beq{
    \Bar{F}_a = \frac{\G(1+\alpha)}{\Tilde{P}_a^\alpha},
    \label{eq:Fbar*}
}
where $\G$ is the Gamma function; see the Appendix. We will refer to this as the ``analytical harm'' in the rest of the paper. The harm incurred for different settings, e.g., a sub-optimal defender distribution $P_d$, can be compared to this quantity.

% We will be interested in measuring the harm due to a sub-optimal defender distribution $P_d$ and will use the total variation distance
% \[
%     \text{TV}(P_d, P_d^*) = \f{1}{2} \norm{P_d - P_d^*}_1
% \]
% to measure the discrepancy between two distributions.

==> v0/problem_robotics.tex <==
% !TEX root = ./root.tex

\section{Problem Formulation}
\label{s:problem}

Consider the problem where a team of $N_a$ attackers attempts to penetrate an area defended by $N_d$ defenders distributed over a its perimeter. Defenders look to position themselves such that they maximize the probability successfully interacting with all attackers. 

All agents have first-order dynamics with bounded speeds and limited control authority. In this problem, these defenders are restricted to only moving along the perimeter of the closed area to block attackers that are initialized on the outside.
% , i.e. we imagine this problem with a defense protecting a circle area with a perimeter supported on [0,1]. 
We normalize the problem space to be dimensionless such that the perimeter has a length, $X=1$, attackers spawn at $Y=1$, and all agents have a speed of $\|u\|\leq 1$.
The problem executes in discrete time with the following agent dynamics
\beq{   \label{eq:dynamics} 
    \Bar{x}_{t+\t} = \Bar{x}_t + \t \Bar{u},
}
 where the agents transition from states $\Bar{x}_t$ to $\Bar{x}_{t+1}$ with controls $\|\Bar{u}\| = 1$ and discrete timestep $\t$. We relate $\t$ such that the perimeter has $N$ number of discrete states. $N$ is a function of the perimeter length $X=1$ such that $N = X/\t$.

Agents move according to the discretized first-order dynamics, where attackers move towards the perimeter and defenders move along the perimeter hoping to capture them. Next, we will describe these teams in terms of discrete probability distributions, how they interact, and finally the harm caused by an attacker. 
% To get a sense of the entire problem, we look at the teams as probability distributions. 
% let us the consider interactions between a defender and an attacker and the penalty the defense receives for failing to recognize the attacker.
% Given this setting, we model the problem such that we can find the optimal repertoire distribution of defenders that best protects the against an attack. To find this distribution we must consider interactions between defender and attacker and the penalty the defense receives for failing to recognize the attacker.

\heading{Definition 1} (Defenders). A team of defenders is distributed over the perimeter $x \in [0,1]$ with $N$ discrete states. Defenders, with dynamics~\cref{eq:dynamics}, move along the perimeter such that the repertoire, at each timestep, can be described by vector $\Bar{p}_d = [p_1,\dots,p_d,\dots,p_{N}]$ where $p_d$ is the number of defenders at location $d$ and $\sum^N_d \Bar{p}_d = N_d$. Let the defender distribution $P_d$ be the discrete probability such that $\sum_d P_d = 1$ and $P_d = \Bar{p}_d/ N_d$.

\heading{Definition 2} (Attackers). A team of attackers is distributed over the state space $x \in [0,1]$ with $N$ discrete states, and initialized at $Y=1$. The attacking team repertoire, at each timestep, is described as the vector $\Bar{q}_a = [q_1, \dots,q_a,\dots, q_{N}]$ where $q_a$ is the number of attackers at location $a$ and $\sum_a^N \Bar{q}_a = N_a$. Let $Q_a$ be attacker distribution, i.e. the probability that an attacker is present at the discrete location $a$ where $Q_a = \Bar{q}_a/N_a$, such that $\sum_a Q_a = 1$. At each timestep, the attackers move synchronously towards the perimeter with constant speed $\|u\|=1$.

\paragraph{Interaction between attackers and defenders} We set up the problem such that defenders have a probability $f_{d,a}$ (which we call the ''cross-reactivity function'') of successfully interacting with an attacker through the use of a sensor with a Bernoulli probability of success. As the defender sits on the perimeter, in its current discrete space $d$, and looks out towards its assigned attacker at $a$, the probability $f_{d,a}$ is calculated according to the Gaussian cross-reactivity function, $f_{d,a} \propto e^{\f{-(d-a)^2}{2\s^2}}$,
where $\s$ is bandwidth of the Gaussian cross-reactivity function.
Cross-reactivity is as a general way of relating an attacker $a$ and a defender $d$. In the Euclidean state space, it depends on the relative position of the defender $d$ and attacker $a$ such that $f_{d,a} = f(d-a)$ where $f$ increases as the distance between $d$ and $a$ decreases. The cross-reactivity function could also be framed in the shape space where $d$ and $a$ denote the type and capabilities of the agent and $\s$ relates the the width between heterogeneous types (we explore that in~\cref{s:heterogeneity}). 

% Given that a defender $d$ is assigned an attacker $a$, 
We can model the interaction between an attacker $a$ and some defender $d$ as a Poisson random variable with rate $\l_a(t)$. Larger the number of attackers, larger the rate of interaction with them; we model this as a rate that increases exponentially with time $\dot{\l}_a(t) = \l_a \nu'_a$ starting from some initial rate $\l_a(0) = 1$ (for sampled $a \sim Q_a$). In biology, this is because the population of pathogens grows. For us it is because the attacker spends more time in the environment.

\paragraph{Harm caused by attackers}
The number of interactions of attacker of type $a$ denoted by $m_a(t)$ also grows exponentially $\dot{m_a}(t) = m_a \nu_a$ starting from some $m_a(0) = 1$ (for sampled $a \sim Q_a$) if it is not captured successfully. The exponents $\nu_a$ and $\nu_a'$ may be different because the number of attackers $a$ that cause harm may grow differently than the number of attackers $a$ that can be observed by the defense. 

The probability of a successful interaction (that leads to capture) can be calculated such that
\[
    \aed{
    \Dot{m}_a(t) &= \text{Poisson}(\l_a)\\
    P(\text{Interaction}) &= e^{-\l_a} \\
    % \begin{cases} 
    %     1 &\text{with prob. } 1- \f{\l_a^0 e^{-\l_a}}{0!}\\  %\text{Pois}(\l_a(t))\\
    %     0 &\text{with prob. } \f{\l_a^0 e^{-\l_a}}{0!}  %\text{Pois}(\l_a(t)).
    % \end{cases}\\
    P(\text{Success}|\text{Interaction}) &= f_{d,a}\\
        % P(\text{Success}) &= 
    % \begin{cases} 
    %     1 &\text{with prob. } f_{d,a}\\
    %     0 &\text{with prob. } 1- f_{d,a}.
    % \end{cases}\\
    P(\text{Success}) =  P(\text{Success}&|\text{Interaction})P(\text{Interaction})
}
\]
Given an attacker distribution, $Q_a$, randomly draw an attacker $a$. The total probability that this attacker $a$ is successfully captured by the defender distribution is $\Tilde{P}_a = \sum_d f_{d,a} P_d$, i.e. the coverage of defender distribution, $P_d$, with its cross-reactivity, $f_{d,a}$, over an attacker $a$. In this problem, we want to position defenders in locations to maximize the $P(\text{Success})$ over all attackers which minimizes the expected number of interactions of an attacker with some defender before being captured, $m_a(t) = \int_0^t \dd{\t} \l_a(\t) \approx \l_a(0) (e^{\nu'_a t - 1})/\nu'_a$.

Unsuccessful interactions of defenders with attackers cause one unit of harm. For large times $t \approx \log(m_a/\l_a(0))/\nu'_a$, the expected harm caused by an attacker of type $a$ after $m$ unsuccessful interactions is
\beq{
    F_a(m) = F_a(0) \rbr{\f{m}{\l_a(0)}}^{\nu_a/\nu'_a} \propto m^\a;
    \label{eq:fm}
}
where $\a = \nu_a/\nu'_a$. The quantity $F_a(m)$ is polynomial in the number of interactions $m$ in this paper but it can also take other forms, e.g., $F_a(m) = 1 - e^{-\b m}$ would model the situation where the harm plateaus after a large number of interactions. The harm $\Bar{F}_a$ caused by an attacker $a$ is thus the average recognition time
\beq{
    \Bar{F}_a = \Tilde{P}_a \int_0^{\infty} \dd{m} F_a(m) e^{-m \Tilde{P}_a}.
    \label{eq:Fbar}
}
We call this the ``empirical harm'' because we will be able to estimate it using simulations.

\paragraph{Minimizing the harm}
The harm caused by an attacker sampled from $Q_a$ is
\beq{
    \text{Harm}(P_d) = \sum_a Q_a \Bar{F}_a.
    \label{eq:harm}
}
It is a function of the defender distribution $P_d$ and our goal will be to minimize it. When $F_a(m) = m^\a$, the optimization problem can be solved analytically to obtain the mean harm
\beq{
    \Bar{F}_a = \frac{\G(1+\alpha)}{\Tilde{P}_a^\alpha},
    \label{eq:Fbar*}
}
where $\G$ is the Gamma function; see the Appendix. We will refer to this as the ``analytical harm'' in the rest of the paper. The harm incurred for different settings, e.g., a sub-optimal defender distribution $P_d$, can be compared to this quantity.

% Given the coverage of the defender repertoire, consider the average harm, $\Bar{F}_a$, the attacker $a$ will cause. We define $\Bar{F}_a(\Tilde{P}_a)$ as a decreasing function of its argument, i.e. more coverage over $a$ decreases the average harm of $a$. Thus, the overall expected harm is the harm averaged over the entire attacker distribution $Q_a$,
% \beq{
%     \text{Harm}(P_d) = \sum_a Q_a \Bar{F}_a (\Tilde{P}_a).
% }
% Thus, the harm is a function of the defender distribution and our job is to choose a $P_d$ that minimizes this objective.


% Discreteness
% Capture sensor/ cross reactivity
% talk about harm. the harm caused is the number of attackers that survive each time step until the game has ended.




==> v0/related.tex <==
% !TEX root = ./root.tex

\section{Discussion and Related Work}
\label{s:related_work}

Pursuit-evasion games have seen a wide range of perspectives~\cite{Karaman2010, isaacs1954}, surveys~\cite{Volkan-PEsurvey,robin:hal-01183372}, and applications such as search and rescue~\cite{Kumar2004} and environmental monitoring~\cite{Dunbabin2012}. Problems with multiple agents are complex due to their high dimensional state-space~\cite{Hilal2013AnIS}. We investigate a variant of the pursuit-evasion game first introduced as the target-guarding problem where the pursuer/defender tries to prevent the evader/intruder from reaching the target~\cite{Garcia-coopdeffrommissiles,Shishika_ReviewPDGames}. A large body of the work on this problem~\cite{Shishika-coopPD2020,VanMoll-turretdefense,Lee-GroundvsAir} studies how multiple defenders decompose the problem into smaller games~\cite{Shishika2018, Macharet-adaptive}, or reduce the defense strategy to an assignment problem~\cite{Chen-ReachAvoid}.

%Classical control has been extended to the multi-agent setting~\cite{fierro-MRCoordination, Sukhatme2008} with some applications such as target tracking/sensing problem~\cite{Salam-adaptivesampling} and localization~\cite{Spletzer-cooplocalization}. A wide array of works have been able to incorporate information-based control as their objectives~\cite{Atanasov-DecAIA,Schlotfeldt-ResilientAIA22,Kantaros-scalableAIA,Tzes-distAIG21,Jeong-RLAIA} for better situational awareness~\cite{Salam-sitawareness}.

A theme that has emerged recently in reinforcement learning-based multi-agent control~\cite{Tan93multi-agentreinforcement, lowe2020multiagent,jeong2020learning} is to obtain decentralized, cooperative policies~\cite{Adler2002,khan2019graph,li2021deep} to tackle non-stationarity and limited information. A popular paradigm is to train a centralized policy and execute it in a decentralized fashion~\cite{WANG2020101,son2019qtran,foerster2017counterfactual,sharma2021survey,terry2020revisiting}. Emergence of coordination has also been studied~\cite{barton2019evaluating,asher2020multi,baker2020emergent}. These methods typically suffer from poor sample complexity but some have been scaled to large problems using heuristics~\cite{khan2018scalable,Low05autonomicmobile,long2020evolutionary}.

This work uses non-learned based methods but demonstrates scalable decentralized policies that can adapt to a wide range of changing attacker distributions for problems as large as 1000 attackers and defenders, albeit in the limited context of a perimeter-defense game. We also obtain a useful guiding principle: competition among the defenders where successful interaction with the attackers acts as the reward may achieve optimality of the resources spent. Such ideas can be used for designing new reinforcement learning methods for multi-agent control. Prior work has noticed the benefits of a similar competition arising out of stochastic policies~\cite{hsu2020scalable}.

Our work is inspired from how the adaptive immune system in humans is organized. We strongly build upon the recent literature in biophysics which models the response of the adaptive immune system in an environment with a large number of evolving pathogens~\cite{MayerRemembers,Mayer8630,Mayer5914}. We believe that the salient traits exhibited in the immune system such as heterogeneous defender types with wide cross-reactivity that interact with a range of attackers, and decentralized estimation and execution are key building blocks for understanding multi-agent autonomy. There are also a number of works that use bio-inspired approaches  mimicking the behavior of ants, bees and flocks~\cite{Hsieh2008BiologicallyIR,Franks2002,Zavlanos-controlforflocking} for multi-agent control.

Broadly speaking, \emph{modeling} heterogeneity has received relatively little interest~\cite{Mitra-HeterogeneityBandit}. Heterogeneity comes in many forms such as differences in roles~\cite{fernandez2021emergent,wang2020roma,Wang-RODE}, robotic capabilities and or sensors~\cite{Salam-heterosensors, shishika-teamcomphetero}, dynamics~\cite{Szwaykowska-heterodynamics,Edwards-heterocontrol}, and even teams of air and ground robots~\cite{chaimowicz-airground,Grocholsky-coopairground}. But algorithmic methods that can tackle large-scale heterogeneity have been difficult to build. This work uses a simple formulation to understand how to devote resources optimally in a heterogeneous environment.
